The Balanced-Pairwise-Affinities Feature Transform

The Balanced-Pairwise-Affinities (BPA) feature transform is designed to upgrade the features of a set of input items to facilitate downstream matching or grouping related tasks. The transformed set encodes a rich representation of high order relations between the input features. A particular min-cost-max-flow fractional matching problem, whose entropy regularized version can be approximated by an optimal transport (OT) optimization, leads to a transform which is efficient, differentiable, equivariant, parameterless and probabilistically interpretable. While the Sinkhorn OT solver has been adapted extensively in many contexts, we use it differently by minimizing the cost between a set of features to $itself$ and using the transport plan's $rows$ as the new representation. Empirically, the transform is highly effective and flexible in its use and consistently improves networks it is inserted into, in a variety of tasks and training schemes. We demonstrate state-of-the-art results in few-shot classification, unsupervised image clustering and person re-identification. Code is available at \url{github.com/DanielShalam/BPA}.

==> implementation_details.tex <==
%=============================================================
\noindent\textbf{Tasks/Applications}: \simon{TBD}
We consider three different applications to evaluate the performance of our method. 

%=============================================================
\noindent\textbf{Performance Measures}: \simon{TBD}
For \emph{few-shot classification} we use...
For \textit{unsupervised image clustering} we use...
For \textit{person re-identification} (ReID) we use...

%=============================================================
\noindent\textbf{Datasets:}
% For \textit{unsupervised clustering} we designed a specialized synthetic data set with the goal of enabling controlled experiments over a wide range of difficulties, which are determined by data dimensionality and in-cluster spread.
For \emph{few-shot classification} we use the standard benchmarks in the literature. The \emph{MiniImagenet} \cite{vinyals2016matching} dataset is a subset of \emph{Imagenet} \cite{Imagenet} that contains 100 classes and 600 images of size 84x84 per class. We follow the standard setup of using 64 classes for training and 16 and 20 novel classes for validation and testing. The \emph{CIFAR-FS} \cite{CIFAR} dataset includes 100 classes with 600 images of size 32 × 32 per-class. We used the same splits as in \emph{MiniImagenet} for this dataset. %The \emph{CUB} \cite{CUB} dataset includes 200 classes of bird species and has 11,788 images of size 84 × 84 pixels in total. We followed the split suggested in \cite{CUBSPLIT} into 100 base classes, 50 validation classes and 50 novel classes.
%
For \textit{unsupervised image clustering} we use three common data-sets, with their standard splits: \emph{STL-10} \cite{coates2011analysis}, \emph{CIFAR-10} and \emph{CIFAR-100-20} \cite{krizhevsky2009learning}. \simon{give details like above?}
%
For \textit{person re-identification} (ReID) we use two common large-scale datasets. The \emph{Market-1501} \cite{Market} and \emph{CUHK03} \cite{CUHK03} dataset consists of 1,501 and 1,467 identities and a total of 32,668 and 14,097 images taken from 6 cameras. 
%
We use the validation and test sets according to the splits in \cite{torchreid}.% \simon{D: Please verify numbers..}

%=============================================================
\noindent\textbf{Pre-training: \simon{Need to say more clearly which experiments this is related to}} We pre-trained ProtoNet~\cite{snell2017prototypical} with a 4-layer Convolution network adapting the procedures of \cite{snell2017prototypical} for training both with and without BPA, training on a 5-way (5/1)-shot 15-query task, using ADAM \cite{kingma2014adam} with learning rate 0.01 and step size of 20 over 100 episodes (tasks) per epoch.


% \vspace{3pt}\noindent\textbf{BPA insertion \textit{without} network retraining}
% (notated by BPA$\blue{_\textit{p}}$ in Tables \ref{tab:results_fsc_MiniImagenet} and \ref{tab:results_fsc_CIFAR_CUB}).
% Recall that the proposed transform is \textit{non-parametric}. As such, we can simply apply it to a trained network at inference, without the need to re-train. This basic `drop-in' use of BPA consistently, and in many cases also significantly, improved the performance of the tested methods, including state-of-the-art, across all benchmarks and backbones. 

% \vspace{3pt}\noindent\textbf{BPA insertion \textit{with} network retraining}
% (notated by BPA$\red{_\textit{t}}$ in Table \ref{tab:results_fsc_MiniImagenet}).
% Due to its \textit{differentiability} property, the proposed method can be applied while training and hence we expect an adaptation of the hosting network's parameters to the presence of the transform with a potential for improvement. 

% \vspace{3pt}\noindent\textbf{inductive BPA insertion \textit{with} with retraining}
% (notated by BPA$\cyan{_\textit{i}}$ in Table \ref{tab:results_fsc_MiniImagenet}).

%=============================================================
\noindent\textbf{Fine-tuning:\simon{Same here..}} We perform fine-tuning on two types of backbone residual networks - a resnet-12 as used in \cite{ye2020few} and a WRN-28-10 as used in \cite{mangla2020charting}.
For ProtoNet~\cite{snell2017prototypical} and ProtoNet-BPA, we fine-tune the base network with parameters taken from \cite{ye2020few}.
For PTMAP-BPA, we use meta-training with batches of a single 10-way 5-shot 15-query task per batch. We use ADAM with learning rate $5e-5$ that decreases with step size 10 for 25 epochs. We train the WRN-28-10 and the resnet-12 backbones for 800 and 100 episodes respectively per epoch.


%=============================================================
%\noindent\textbf{Pairwise distance metric:} When using a pre-trained network, the distance metric used by BPA should be related to the original distance metric. Therefore, we use unnormalized Euclidean distances in works like ProtoNet \cite{snell2017prototypical} which do not normalize in pre-training.
